Coordinate Ascent for Off-Policy RL with Global Convergence Guarantees

We revisit the domain of off-policy policy optimization in RL from the perspective of coordinate ascent. One commonly-used approach is to leverage the off-policy policy gradient to optimize a surrogate objective -- the total discounted in expectation return of the target policy with respect to the state distribution of the behavior policy. However, this approach has been shown to suffer from the distribution mismatch issue, and therefore significant efforts are needed for correcting this mismatch either via state distribution correction or a counterfactual method. In this paper, we rethink off-policy learning via Coordinate Ascent Policy Optimization (CAPO), an off-policy actor-critic algorithm that decouples policy improvement from the state distribution of the behavior policy without using the policy gradient. This design obviates the need for distribution correction or importance sampling in the policy improvement step of off-policy policy gradient. We establish the global convergence of CAPO with general coordinate selection and then further quantify the convergence rates of several instances of CAPO with popular coordinate selection rules, including the cyclic and the randomized variants of CAPO. We then extend CAPO to neural policies for a more practical implementation. Through experiments, we demonstrate that CAPO provides a competitive approach to RL in practice.

==> 3-SGD.tex <==
\section{The Effect of Stochasticity in Policy Gradient}
\label{section:SGD}
While it has been shown that exact NPG converges to the global optimum \cite{agarwal2020theory, bhandari2019global}, such property is not reserved under the stochastic setting. \citep{chung2020variance, mei2021understanding} argued that due to the vicious cycle of on-policy sampling, NPG will converge to local optimum with positive probability.

\subsection{Setting: Multi-Arm Bandit}
\label{SGD:multi-arm-bandit}
We consider a deterministic K-arm bandit with single state and action set $a \in \left[K\right]$ and a softmax policy $\pi_{\theta}: [K] \rightarrow [0, 1]$, the reward vector $r \in \mathbb{R}^{K}$ is the reward corresponding to each action. This setting is the same as the one in \textbf{Section 2.} \citet{mei2021understanding}, where we also assume that the reward is positive such that $r(a) \in [0, 1), \forall a \in [K]$.

Our goal here is to find the optimal policy $\pi^{*}$ that maximize the expected total reward, since there is only one single state, the objective function can by written as:
\begin{equation}
%
J(\theta) = \mathbb{E}_{{a \sim \pi_{\theta}(\cdot)}}[r(a)]
%
\end{equation}

\subsection{Stochastic Policy Gradient with Importance Sampling}
\citet{mei2021understanding} has showed that by using the importance sampling (IS) reward estimator $\hat{r}_{t}(a)$:
\begin{equation}
\hat{r}_{m}(a)=\frac{\mathbb{I}\left\{a_{m}=a\right\}}{\pi_{\theta_{m}}(a)} \cdot r(a) \text { for all } a \in[K] 
\end{equation}

the stochastic policy gradient with IS update (\eqref{eq:is_spg_update}) converges to global optimum with probability: 
\begin{equation}
\label{eq:is_spg_update}
\theta_{m+1} \longleftarrow \theta_{m}+\eta \cdot \frac{d \pi_{m}^{\top} \hat{r}_{m}}{d \theta_{m}},
%
\text{where }
\frac{d \pi_{m}^{\top} \hat{r}_{m}}{d \theta_{m}(a)} =
\pi_{m}(a) \cdot\left(\hat{r}_{m}(a)-\pi_{m}^{\top} \hat{r}_{m}\right)
\end{equation}

\subsection{Vanilla Stochastic Policy Gradient}
However, another unbiased estimator of PG (\eqref{eq:spg_update}) that does not utilize the IS reward estimator is more wildly used:
\begin{equation}
\label{eq:spg_update}
\theta_{m+1} \longleftarrow \theta_{m}+\eta \cdot \frac{d \pi_{m}^{\top} r}{d \theta_{m}},
%
\text{where }
\frac{d \pi_{\theta_{m}}^{\top} r}{d \theta_{m}(a^{\prime})} =
%
(\mathbb{I}\left[a=a^{\prime}\right] - \pi_{m}(a^{\prime})) \cdot \left(r(a)\right)
\end{equation}

%
\begin{theorem} With positive probability, $\sum_{a \neq a^{*}} \pi_{\theta_m} \rightarrow 1$ as $m \rightarrow \infty$ under the vanilla stochastic policy update (\eqref{eq:spg_update}).
\label{theorem:on_pg_stuck}

The proof can be found in Appendix \ref{app:on_pg}, the idea is that early update toward the sub-optimal action will increase the probability of visiting such sub-optimal action in the future iterations. This vicious cycle of on-policy sampling will cause the policy to become deterministic too fast, the inability of SPG to escape from the local optimum then directly cause the policy to stuck at local.

Theorem \ref{theorem:on_pg_stuck} shows that \eqref{eq:spg_update}, unlike its IS twin \eqref{eq:is_spg_update}, can stuck in local optimum.
Two main problems can be observed:
\vspace{-2mm}
\begin{itemize}[leftmargin=*]
  \vspace{-1mm}
  \item On-policy sampling will be guided by early updates, thus causing potential early commitment to sub-optimal actions.
  %
  \vspace{-1mm}
  \item Beside the commitment to sub-optimal actions, the inability to escape from the local optimum is another cause that PG will stuck in the local optimum.
\end{itemize}
\end{theorem}

To address the above two problems, we introduce an off-policy actor-critic method Off-CAPO in section \ref{section:method} to avoid the vicious cycle from on-policy sampling. Moreover, with a well-designed learning rate that allows CAPO to escape from the local optimum, we show that even under the on-policy setting can guarantee global convergence in section \ref{section:method:onCAPO}.


